When Bidders Are DAOs

In a typical decentralized autonomous organization (DAO), people organize themselves into a group that is programmatically managed. DAOs can act as bidders in auctions, with a DAO's bid treated by the auctioneer as if it had been submitted by an individual, without regard to the internal structure of the DAO. We study auctions in which the bidders are DAOs. More precisely, we consider the design of two-level auctions in which the "participants" are groups of bidders rather than individuals. Bidders form DAOs to pool resources, but must then also negotiate the terms by which the DAO's winnings are shared. We model the outcome of a DAO's negotiations by an aggregation function (which aggregates DAO members' bids into a single group bid), and a budget-balanced cost-sharing mechanism (that determines DAO members' access to the DAO's allocation and distributes the total payment demanded from the DAO to its members). We pursue two-level mechanisms that are incentive-compatible (with truthful bidding a dominant strategy for members of each DAO) and approximately welfare-optimal. We prove that, even in the case of a single-item auction, incentive-compatible welfare maximization is not possible: No matter what the outer mechanism and the cost-sharing mechanisms used by DAOs, the welfare of the resulting two-level mechanism can be a $\approx \ln n$ factor less than optimal. We complement this lower bound with a natural two-level mechanism that achieves a matching approximate welfare guarantee. Our upper bound also extends to multi-item auctions where individuals have additive valuations. Finally, we show that our positive results cannot be extended much further: Even in multi-item settings with unit-demand bidders, truthful two-level mechanisms form a highly restricted class and as a consequence cannot guarantee any non-trivial approximation of the maximum social welfare.

==> notations.tex <==
\newcommand{\highest}{D_{j*}}
\newcommand{\second}{D_{j'}}

\newcommand{\dao}[1]{G_{#1}}
\newcommand{\leader}[1]{L_{#1}}

\newcommand{\mech}{\mathcal{M}}
\newcommand{\lowermech}{\mathcal{M}_l}
\newcommand{\uppermech}{\mathcal{M}_u}
\newcommand{{\biddingLang}}{\mathcal{B}}

\newcommand{\upperal}{x^u}
\newcommand{\loweral}{x^l}

\newcommand{\OPT}{\texttt{OPT}} 
